Probing compressed mass spectra in electroweak supersymmetry with Recursive Jigsaw Reconstruction

The lack of evidence for the production of colored supersymmetric particles at the LHC has increased interest in searches for superpartners of the electroweak SM gauge bosons, namely the neutralinos and charginos. These are challenging due to the weak nature of the production process, and the existing discovery reach has significant gaps in due to the difficulty of separating the supersymmetric signal from SM diboson events that produce similar final states and kinematics. We apply the Recursive Jigsaw Reconstruction technique to study final states enriched in charged leptons and missing transverse momentum, focusing on compressed topologies with direct production of charginos and neutralinos decaying to the lightest neutral supersymmetric particle through the emission of W and Z bosons. After presenting prototype analysis designs for future LHC runs, we demonstrate that its detectors have the potential to probe a significant amount of unexplored parameter space for chargino-neutralino associated production within the next few years, and show that the very challenging successful search for chargino pair production with compressed spectra might be possible by the end of the LHC lifetime.

==> Makefile <==
# Makefile for creating an ATLAS LaTeX document
#------------------------------------------------------------------------------
# By default makes mydocument.pdf using target run_pdflatex
# Replace mydocument with your main filename or add another target set
# Replace BIBTEX = bibtex with BIBTEX = biber if you use biblatex and biber instead of bibtex
# Use "make clean" to cleanup.
# "make cleanall" also deletes the PDF file $(BASENAME).pdf.

LATEX    = latex
PDFLATEX = pdflatex
BIBTEX   = bibtex
# BIBTEX   = biblatex
#BIBTEX = biber
DVIPS    = dvips
DVIPDF   = dvipdf

BASENAME = EWKino

# Default target - make mydocument.pdf with pdflatex
default: run_pdflatex


run_pdflatex: $(BASENAME).pdf
	@echo "Made $<"

run_latex: $(BASENAME).dvi
	$(DVIPDF) -sPAPERSIZE=a4 -dPDFSETTINGS=/prepress ${BASENAME}
	@echo "Made $<"

# Standard Latex targets
%.pdf:	%.tex *.bib
	pdflatex  -shell-escape ${BASENAME}
	pdflatex  -shell-escape ${BASENAME}
	$(BIBTEX) ${BASENAME} 
	pdflatex  -shell-escape ${BASENAME}
	pdflatex  -shell-escape ${BASENAME}

%.dvi:	%.tex 
	$(LATEX)    $<
	$(BIBTEX)   $(basename $<)
	$(LATEX)    $<
	$(LATEX)    $<

%.bbl:	%.tex *.bib
	$(LATEX) $*
	$(BIBTEX) $*


%.ps:	%.dvi
	$(DVIPS) $< -o $@

clean:
	-rm *.dvi *.toc *.aux *.log *.out \
		*.bbl *.blg *.pdf

cleanpdf:
	-rm $(BASENAME).pdf 


cleanall: clean cleanpdf
	-rm $(BASENAME).pdf 


